An Introduction to Neural Data Compression

Neural compression is the application of neural networks and other machine learning methods to data compression. Recent advances in statistical machine learning have opened up new possibilities for data compression, allowing compression algorithms to be learned end-to-end from data using powerful generative models such as normalizing flows, variational autoencoders, diffusion probabilistic models, and generative adversarial networks. The present article aims to introduce this field of research to a broader machine learning audience by reviewing the necessary background in information theory (e.g., entropy coding, rate-distortion theory) and computer vision (e.g., image quality assessment, perceptual metrics), and providing a curated guide through the essential ideas and methods in the literature thus far.

==> CGV-107-nowbook.tex <==
\PassOptionsToClass {book,biber}{nowfnt}
\input {CGV-107}


==> CGV-107-nowchapter.tex <==
\PassOptionsToClass {chapter,biber}{nowfnt}
\input {CGV-107}


==> CGV-107-nowebook.tex <==
\PassOptionsToClass {ebook,biber}{nowfnt}
\input {CGV-107}


==> CGV-107-nowechapter.tex <==
\PassOptionsToClass {echapter,biber}{nowfnt}
\input {CGV-107}


==> CGV-107-nowplain.tex <==
\PassOptionsToClass {plain,biber}{nowfnt}
\input {CGV-107}


==> CGV-107-nowsample.tex <==
\PassOptionsToClass {sample,biber}{nowfnt}
\input {CGV-107}


==> CGV-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Aaron Hertzmann }{Adobe Research, USA}


\subsection{Editors} \scriptsize
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Marc Alexa}{TU Berlin}
\journaleditor{Kavita Bala}{Cornel}
\journaleditor{Ronen Basri}{Weizmann Institute of Science}
\journaleditor{Peter Belhumeur}{Columbia University}
\journaleditor{Andrew Blake}{Microsoft Research}
\journaleditor{Chris Bregler}{Facebook-Oculus}
\journaleditor{Joachim Buhmann}{ETH Zurich}
\journaleditor{Michael Cohen}{Facebook}
\journaleditor{Brian Curless}{University of Washington}
\journaleditor{Paul Debevec}{USC Institute for Creative Technologies}
\journaleditor{Julie Dorsey}{Yale}
\journaleditor{Fredo Durand}{MIT}
\journaleditor{Olivier Faugeras}{INRIA}
\journaleditor{Rob Fergus}{NYU}
\journaleditor{William T. Freeman}{MIT}
\journaleditor{Mike Gleicher}{University of Wisconsin}
\journaleditor{Richard Hartley}{Australian National University}
\journaleditor{Hugues Hoppe}{Microsoft Research}
\journaleditor{C. Karen Liu}{Stanford}
\journaleditor{David Lowe}{University of British Columbia}
\journaleditor{Jitendra Malik}{ Berkeley}
\journaleditor{Steve Marschner}{Cornell}
\journaleditor{Shree Nayar}{Columbia}
\journaleditor{Tomas Pajdla}{Czech Technical University}
\journaleditor{Pietro Perona}{California Institute of Technology}
\journaleditor{Marc Pollefeys}{ETH Zurich}
\journaleditor{Jean Ponce}{Ecole Normale Superieure}
\journaleditor{Long Quan}{HKUST}
\journaleditor{Cordelia Schmid}{INRIA}
\journaleditor{Steve Seitz}{University of Washington}
\journaleditor{Amnon Shashua}{Hebrew University}
\journaleditor{Peter Shirley}{University of Utah}
\journaleditor{Noah Snavely}{Cornell}
\journaleditor{Stefano Soatto}{UCLA}
\journaleditor{Richard Szeliski}{Microsoft Research}
\journaleditor{Luc Van Gool}{KU Leuven and ETH Zurich}
\journaleditor{Joachim Weickert}{Saarland University}
\journaleditor{Song Chun Zhu}{UCLA}
\journaleditor{Andrew Zisserman}{Oxford}
\end{multicols*}
\end{editorialboard} 

==> CGV-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{CGVcolor}{cobalt}   %
\journalcolor      {CGVcolor} %
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Computer Graphics and Vision}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {CGV}
\journalurl        {http://www.nowpublishers.com/CGV}
\journalissnprint  {1572-2740}
\journalissnonline {1572-2759}
\journaldoi        {10.1561/06}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} %

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Rendering}
\item{Shape}
\item{Mesh simplification}
\item{Animation}
\item{Sensors and sensing}
\item{Image restoration and enhancement}
\item{Segmentation and grouping}
\item{Feature detection and selection}
\item{Color processing}
\item{Texture analysis and synthesis}
\item{Illumination and reflectance modeling}
\item{Shape representation}
\item{Tracking}
\item{Calibration}
\item{Structure from motion}
\item{Motion estimation and registration}
\item{Stereo matching and reconstruction}
\item{3D reconstruction and image-based modeling}
\item{Learning and statistical methods}
\item{Appearance-based matching}
\item{Object and scene recognition}
\item{Face detection and recognition}
\item{Activity and gesture recognition}
\item{Image and video retrieval}
\item{Video analysis and event recognition}
\item{Medical image analysis}
\item{Robot localization and navigation}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Computer Vision for Autonomous Vehicles: Problems, Datasets and State of the Art}\\
Joel Janai, Fatma Güney, Aseem Behl and Andreas Geiger\\
ISBN: 978-1-68083-688-2\\
\\
\noindent \textit{Discrete Graphical Models - An Optimization Perspective}\\
Bogdan Savchynskyy\\
ISBN: 978-1-68083-638-7\\
\\
\noindent \textit{Line Drawings from 3D Models: A Tutorial}\\
Pierre Bénard and Aaron Hertzmann\\
ISBN: 978-1-68083-590-8\\
\\
\noindent \textit{Publishing and Consuming 3D Content on the Web: A Survey}\\
Marco Potenziani, Marco Callieri, Matteo Dellepiane and Roberto Scopigno\\
ISBN: 978-1-68083-536-6\\
\\
\noindent \textit{Crowdsourcing in Computer Vision}\\
Adriana Kovashka, Olga Russakovsky, Li Fei-Fei and Kristen Grauman\\
ISBN: 978-1-68083-212-9\\
\\
\noindent \textit{The Path to Path-Traced Movies}\\
Per H. Christensen and Wojciech Jarosz\\
ISBN: 978-1-68083-210-5\\
\\
\noindent \textit{(Hyper)-Graphs Inference through Convex Relaxations and Move Making Algorithms}\\
Nikos Komodakis, M. Pawan Kumar and Nikos Paragios\\
ISBN: 978-1-68083-138-2\\


==> NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}
